Dynamical stability of 2D topological lasers

In this internship report, I have considered the topological laser built by amplifying the edge of a 2D Harper-Hofstadter photonic lattice, with the reservoir of carriers being treated explicitly. The dynamical stability of the resulting chiral laser operation is investigated by means of the Bogoliubov approach on top of the lasing state. In particular, I propose a mapping to the 1D model of a standard laser which captures the main features of the slow decaying Goldstone mode. Also, instabilities arising from the interplay of chiral propagation with refractive index nonlinearities and the non-adiabatic reservoir of carriers are highlighted.

==> chapters/chapter00_abstract.tex <==
\chapter*{Resumen}




==> chapters/chapter051.tex <==
\chapter{Addition of a nonlinear interaction}


In this chapter, we want to compare the 1D and 2D models when a non-linear term $g|\psi|^2$ is added. From the 1D model, we do not expect any particular phenomena about stability, as long as the sign of the effective mass is the same as the sign of the non-linear strength. The only feature that we expect is that the system become faster as the coupling constant $g$ is raised due to the $\mu'$ factor in (\ref{eq:3.7}).


\section{1D-2D comparison}

For simplicity sake, we consider a system in the adiabatic approximation ($\gamma_R/\gamma= +\infty$), small pump intensity $P^{eff}= 1.25\gamma$, maximal gain wavevector $k_{y0} = -0.9195$ for $N_y=41$ and low value of loss rate ($\gamma/J=0.1$) so that all the blue-shift is due to the non-linear term.

This time, we use a seed to lase at the wanted wavector with $g=0$. Then we use the SS of this simulation as the initial condition for simulations with $g=0.001$ and $g=-0.0025$. We do the same with the SS of $g=0.001$ to obtain the SS for higher values of $g$.

\textit{Results}:

Some results of this simulation are shown in Fig. \ref{fig5.1}. In Fig. \ref{fig5.1} (a), we display the dispersion indicating with a dark line the lasing states studied. In Fig. \ref{fig5.1} (b), we show that the effective mass of the lasing mode (black dot) is positive. In Fig. \ref{fig5.1} (c),(d), we can see the real and imaginary part of the elementary excitations spectrum. As it corresponds to a negative non-linear term, we find that the state is unstable. To get this result with the 2D model, we started with the SS of the $g=0$ simulation, and then rose $g$ to $-0.025$. The system reached the new SS quickly, a little before being destabilized by noise. Thus we extracted the wavefunction of the system during this short stable period to plot the elementary excitation spectrum. The slight discrepancy between 1D and 2D model may be due to the fact that the state is already a bit unstable, as we see that the Golstone theorem is already weakly broken (the $k=0$ value of the Goldstone mode is different from 0).

In Fig. \ref{fig5.1} (e)-(h), we see the elementary excitations spectrum of the system for $g=0.001$ and $g=0.0035$. The agreement between the 1D and 2D model is very good in both cases. We also see that the zone of flatness of the Goldstone mode gets narrower when $g$ is raised, as expected from the adiabatic approximation analytical model. 

Finally, we stress that the random choice of chirality is broken when a non-linear term is added. Indeed, one chirality corresponds to an effective mass of opposite sign to the one of the non-linear strength term. This means that the system starts lasing every time in the same gap. 



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.65]{chapters/g_recap.png}
    \caption{Comparison between the 1D and the 2D models elementary excitations spectrum varying the non-linear strength $g$. 
    System parameters: $k_{y,0} = -0.919$, $\mu_T/J = -1.939$, $a_1/J= 1.2310 $, $a_2/J= 0.6179$, $a_3/J= -0.2138$, $a_4/J = -0.1566$, $P^{eff}= 1.25\gamma$, $P^{eff}_{th}= 1.142\gamma$, $\gamma/J= 0.1$, $\beta= 0.01$, $\gamma^{(2)}/J= 0.014$, $N_x=31$, $N_y=41$, adiabatic approximation.
    (a) Zoom on the edge mode dispersion. The red line corresponds to the wavevector for all the simulations. The black horizontal lines show the frequencies of the lasing modes studied. (b) Second derivative of the edge dispersion. The black marker indicates the value of the $a_2$ coefficient corresponding to the lasing modes studied.  
    (c)-(h) Real and imaginary part of the elementary excitation spectrum for the 1D (red) and 2D (black) model as a function of the wave vector $k= k_y - k_{y,0}$ for increasing values of the lasing state wavevector $k_{y,0}$. The zoom is made around $k=0$ since the 1D model is only relevant in this region.
    (c),(d) Real and imaginary part of the spectrum for $g=-0.0025$, corresponding to the bottom black bar in (a). (e),(f) Same for $g=0.001$, corresponding to the middle black bar in (a). (g),(h) Same for $g= 0.035$, corresponding to the top black bar in (a).
    }
    \label{fig5.1}
\end{figure}



\newpage

\section{Reverse chirality instability}

In the previous section, we saw that the agreement between the 1D and 2D model is very good up to a value of $\mu / J = 0.211$, which represents roughly $10\%$ of the gap. This is already a great amount, but it is legitimate to wonder what happens when this is risen up. 

We can do this by raising $g$ to higher values. However, above $g=0.035$, it becomes quickly difficult to get a SS, what is not expected according to the 1D model. 



\begin{figure}[H]   
\begin{minipage}[t]{0.4\textwidth}
Actually, the origin of these instabilities has to be found in the full 2D model, as we can see in Fig. \ref{fig5.2}. We see on this figure that the particle and antiparticle modes corresponding to the mode of opposite chirality on the same edge are very close from the instability threshold. The instability threshold is thus little above $g=0.035$.
\end{minipage}
\begin{minipage}[t]{0.6\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.85]{chapters/high_g_instabilities.png}}
\end{minipage} 

   \caption{Imaginary part of the elementary excitations spectrum for the lasing point \{ $k_{y,0} = -0.9195$, $\mu_T/J = -1.728$\} as a function of the wavevector $k$ computed with the 2D model. System parameters: $g=0.035$, $g_R=0$, $P^{eff}= 1.25\gamma$, $P^{eff}_{th}= 1.142\gamma$, $\gamma/J= 0.1$, $\beta= 0.01$, $\gamma^{(2)}/J= 0.014$, $N_x=31$, $N_y=41$, adiabatic approximation.}
    \label{fig5.2}   
\end{figure} 

In order to proof that our computation of the elementary excitation spectrum is valid, we can probe this instability in another way. We take as initial SS the one got from the previous $g=0.01$ simulation perturbed with a small random noise. We then raise $g$ to $g=0.055$, which we guess is above threshold. We see clearly in Fig. \ref{fig5.3} (a) that the system first want to stabilize in the SS for the new value of $g$ but is unable to damp the growing perturbation. The frequencies involved in this growing perturbation are displayed in Fig. \ref{fig5.3} (b) what confirms that the instability is due to modes in the top gap thus having a reverse chirality compared to the lasing mode. Note that as these modes are themselves unstable, the system becomes fully unstable. 


\begin{figure}[H]
    \centering
    \includegraphics[scale=0.55]{chapters/instability_g_2.png}
    \caption{Time (a) and fourier (b) evolution of a edge site just above instability threshold ($g=0.055$). Other parameters are the same as in Fig. \ref{fig5.2}. In (b), the white (grey) background stands for the gaps (bulk). 
    }
    \label{fig5.3}
\end{figure}



\newpage

\section{Bulk instabilities}

Another way to increase the blue-shift due to the non-linear term is to increase the pump intensity. Indeed in the adiabatic approximation, the blue-shift is quantified by $\mu = g |\psi|^2$, where $|\psi|^2$ increases linearly with the pump intensity. Starting from the SS obtained for $g=0.01$ and $P^{eff} = 1.25\gamma$, then turning to $P^{eff} = 2.15\gamma$, we computed the elementary excitation spectrum on top of the new SS, as in Fig. \ref{fig5.4}.  

\begin{figure}[H]   
\begin{minipage}[t]{0.5\textwidth}
We see on this figure that some modes arising from the bulk are getting very close from the instability threshold, and cross it for a slightly bigger pump intensity. The origin of this new kind of instabilities seems to be the coupling between modes in the bulk induced by the non-linear term and enhanced by the pumping. {\color{red} One explication could be that at high pump intensity there is a strong blue-shift, so the energy of the lasing edge mode gets closer from the energies of some bulk modes, which may favour their excitation.} 
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.85]{chapters/intensity_intability_g.png}}
\end{minipage} 

   \caption{Imaginary part of the elementary excitations spectrum for the lasing point \{ $k_{y,0} = -0.9195$, $\mu_T/J = -1.347$\} as a function of the wavevector $k$ computed with the 2D model. System parameters: $g=0.01$, $g_R=0$, $P^{eff}= 2.15\gamma$, $P^{eff}_{th}= 1.142\gamma$, $\gamma/J= 0.1$, $\beta= 0.01$, $\gamma^{(2)}/J= 0.014$, $N_x=31$, $N_y=41$, adiabatic approximation.}
    \label{fig5.4}   
\end{figure} 


Again, we probe this instability by turning the pump intensity to $P^{eff}= 2.20\gamma$, which is expected to be just above the instability threshold, starting from a stable SS (for $g=0.01$) perturbed with a random noise. We see in Fig. \ref{fig5.5} (a) that the system reaches the new SS meanwhile the perturbation is growing slowly. At a certain point, the perturbation seems to reach a stable cycle (around $T=2000$). In Fig. \ref{fig5.5} (b), we computed the Fourier transform of the signal on the edge within the time frame in the white zone of Fig. \ref{fig5.5} (a). This shows that the system is perturbed by two modes symmetrical around the lasing mode, that are gaining in amplitude with time (not showed). In the steady unstable regime, other modes are further excited due to the instability of the bulk modes perturbing the system. Finally, we can check that the modes that are excited by the perturbation are the one predicted by the elementary excitation spectrum looking at the inset of Fig. \ref{fig5.5} (a), which shows the imaginary part of the excitation spectrum as a function of its real part, thus with the same $x$-axis as the fourier transform.



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.35]{chapters/instability_P_g.png}
    \caption{Time (a) and fourier (b) evolution of a edge site just above instability threshold ($P^{eff}= 2.20\gamma$). Other parameters are the same as in Fig. \ref{fig5.4}. In (a), the white background between the dashed line corresponds to the time frame on which the Fourier Transform (FT) in (b) is computed. Inset: imaginary part of the elementary excitation spectrum of Fig. \ref{fig5.4} as a function of its real part.
    }
    \label{fig5.5}
\end{figure}


\section{Conclusion}

In this chapter, we first checked that the 1D and 2D models agree for small $k$ values, and found satisfying results. However, we discovered new instabilities that cannot be captured with the 1D model. One new source of instabilities is related to the use of a big non-linear strength $g$ at low pumping power, and involve modes in the other gap, namely edge modes with reverse chirality. {\color{red}The mechanism of enhancement of these modes cannot be explained through a momentum dependent loss term as in Chapter \textbf{4} Section \textbf{3}, and is still not understood.} The other new source of instabilities is at moderate non-linear strength $g$ but with high pump intensity. In this case, bulk modes are enhanced and destabilize the system.



==> chapters/chapter06.tex <==
\chapter{1D model with whole edge pumping on a cylinder}

In this chapter, we introduce a very simple model to describe the spatio-temporal evolution of a lasing edge mode. We use it to calculate the elementary excitations, and then compare our results to the findings of recent papers. Finally, we calculate the spatial correlations of this new type of non-equilibrium condensate.

\section{Approximations}

\textit{Cylindrical geometry:}

In real space, a chiral edge mode propagates unidirectionally around the edge. Further, the topological protection makes that a chiral edge mode is not affected by little geometrical perturbations. Thus, a chiral edge mode propagates the same way on different geometries of the edge. In particular, the propagation of a chiral edge state along a square or a circular edge has to be similar. This is why in the following we will consider a cylindrical lattice, namely a lattice with PBC along the $y$-axis, and focus on the chiral edge states on one edge of the lattice (the $x=0$ edge). This way, the results we get should be directly applicable to the square geometry used in the articles of the last chapter, and we can take advantage of the translationnal invariance along the $y$-axis when pumping is homogeneous on the edge.

\textit{Dispersion approximation:}

From the previous approximation, and considering homogeneous pumping along the $x=0$ edge, the Bloch wavevector becomes a good quantum number and the energy bands of the system are the one showed in Fig. \ref{fig2.1}. Thus a lasing chiral edge mode corresponds to a given point ($k_{y,0}$, $w_0$) on this figure. In the following we will consider that the only 

\section{The model}

We place in a cylinder geometry. In real space, a chiral edge mode propagates unidirectionally around one edge (whose direction is fixed by the sign of the group velocity of the dispersion), with a small penetration in the bulk. We thus perform a 1-dimensional approximation of the state neglecting this penetration. The validity of this approximation will be discussed latter in section 3.2. Then, we use the same formalism as \cite{wouters2007excitations} namely a mean-field description of the non-equilibrium condensate in terms of a generalized Gross-Pitaevskii equation (gGPE) with reservoir for the macroscopic lasing state wave function $\psi_n(t) e^{-i(\mu_T t - k_{y,0}n)}$ at frequency $\mu_T$ and wavevector $k_{y,0}$, including loss and amplification terms :

\begin{equation}\label{eq:3.1}
    i\frac{\partial \psi_n}{\partial t} = \Big[w_0 + TF^{-1}[\epsilon(k)](n) \circledast + g|\psi_n|^2 + g_R N_n + i(R N_{n} - \gamma) \Big] \psi_n
\end{equation}

where the reservoir density is determined by the rate equation

\begin{equation}\label{eq:3.2}
      \frac{\partial N_{n}}{\partial t} = P - (\gamma_R + R|\psi_n|^2)N_{n} 
\end{equation}

and $\epsilon(k= k_y - k_{y,0})= a_1 k + a_2 k^2 + a_3 k^3  + a_4 k^4$ is the dispersion around of the lasing edge mode approximated at the first orders, $TF^{-1}$ denotes the inverse fourier transform, $\circledast$ the convolution product, $g$ the strength of the interaction between 2 particles in the lasing mode, $g_R$ is the interaction strength of the interaction between a particle in the lasing mode and a particle in the reservoir, R is the amplification term, $\gamma$ is the on-site loss rate, $\gamma_R$ is the reservoir loss rate, $w_0$ is the bare HH frequency and $P$ the pump that is assumed to be uniform. 

\section{Effective parameters}

\begin{figure}[H]   
\begin{minipage}[t]{0.5\textwidth}
 Actually, the 1D approximation that we made is not totally legitimate. Indeed, the localization of the edge modes is not fully on the last site of the edge, as we can see in Fig. \ref{fig3.1}. With the parameters of this figure, we calculate the inverse participation ratio equals to $1.29$, which we assume is a good estimate whatever are the parameters. We see with this value that it is small but not negligible.
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.5]{chapters/penetration_bulk.png}}
    \caption{Intensity along the transverse direction ($x$-axis). Parameters: $N_x=11$, $k_{y0}= -0.9195$, $w_0/J= -1.9396$, $\mu/J=0$, $\gamma/J=0,1$, $\beta=0.01$, $P=1.25\gamma$}
    \label{fig3.1}
\end{minipage}      
\end{figure}



In order to get quantitative results, we can modify a bit the model exposed in the last section. Penetration in the bulk means that the edge sites in the 2D lattice have a lower intensity compared to the 1D case with same parameters. It is as if the edge site in the 1D case was less pumped. The most simple parameter that characterizes the penetration in the bulk is the ratio $\frac{P_{th}}{\gamma}$, which is the ratio between the pumping threshold (as calculated in section 2.3) of the 2D lattice and the one of the 1D model (equals to the threshold of a single site). So the equivalent pumping term for the 1D model is $P_{eq\ 1D}= \frac{P \gamma}{P_{th}}$ (it is like considering that the losses in the bulk are the same at threshold as over threshold).

Another parameter that can be introduced to get more quantitative results is a momentum dependent loss rate. It is a parameter common in systems described by a gGPE equation like polaritons \cite{baboux2018unstable}, and can have several origins. In our case, as we pump on the edge, we give gain to the modes that are situated on the edge, so the ones around the lasing mode, that correspond to small $k$ modes. On the contrary, modes with bigger $k$ are situated in the bulk and get little gain, so are quickly damped. We can model this phenomenon introducing a momentum dependent loss rate with the form $\gamma_{tot}(k) = \gamma - \gamma^{(2)} k^2$, which is the simplest symmetric form. As $\gamma^{(2)}$ is a parameter a bit tricky to estimate and not fundamental for our purpose, we will give it an arbitrary value or fit it when possible.  

Finally, we will see in the following that these two effective parameters are sufficient to get quantitative results with this 1D model.



\section{Elementary excitations in the general case}

The density uniform steady-state (SS) solution $\psi_n(t) = \psi^0 e^{-i\mu_T t}e^{i k_{y,0}n}$ and $N_n(t)=N^0=\frac{\gamma}{R}$ where $\psi^0 = \sqrt{\frac{\gamma_R}{R}(\frac{P}{P_{th}}-1)}$ (we can choose the phase so that this term is real) and $\mu_T = w_0 + g|\psi^0|^2 + g_R N^0$ is reached above the pump threshold $P^{1D}_{th} = \frac{\gamma \gamma_R}{R}$.



The elementary excitation spectrum is calculated by linearizing (\ref{eq:3.1}) and (\ref{eq:3.2}) around this SS taking the ansatz $\psi_n(t) = \psi^0(1 + \delta \psi_n(t)) e^{-i\mu_T t}e^{i k_{y,0}n}$ and $N_n(t) = N^0 (1 + \delta N_n(t))$ with $\delta\psi_n , \delta N_n \ll 1$ \cite{wouters2007excitations, chiocchetta2013non}. Keeping only terms to first order in $\delta \psi_n$ and $\delta N_n$, and Fourier transforming the spatial coordinate we obtain the motion equations in a matricial form:

\begin{equation}\label{eq:3.3}
i\frac{\partial }{\partial t}&       
\begin{pmatrix} 
        \delta\psi_k \\ 
        \delta\psi_{-k}^{\ast} \\
        \delta N_k
      \end{pmatrix} 
      = \\
     \begin{pmatrix}
    \epsilon(k) + \mu  & \mu  &  \sigma + i \gamma\\
    -\mu & -\epsilon(-k)^* - \mu & -\sigma + i \gamma\\
    -i \alpha \gamma_R & -i \alpha \gamma_R & -i (\alpha +1) \gamma_R
    \end{pmatrix}
    \begin{pmatrix} 
        \delta\psi_k \\ 
        \delta\psi_{-k}^{\ast} \\
        \delta N_k
      \end{pmatrix} 
\end{equation}

where $\mu= g|\psi^0|^2$, $\sigma = g_R N^0 = \frac{g_R \gamma \mu}{\alpha \gamma_R}$ and $\alpha = (\frac{P}{P_{th}}-1)$. Note that this $P$ corresponds to the 2D one.

\vspace{0.25 cm}

Diagonalizing this matrix for each k gives us the elementary excitation spectrum, whose typical examples are shown in Fig. \ref{fig3.2}. In this figure, all the spectrums are calculated at the same lasing point.The results of Fig.\ref{fig3.2}(c),(d) show the spectrum in a system without reservoir and non non-linear interactions, thus similar to the one studied in \cite{secli2019theory}. It shows a slow dynamic around $k=0$ of the Goldstone mode (indicated as $G$), which means that a perturbation in the system with a frequency close to the lasing mode has a long damping time. That is in qualitative agreement with the observations made in \cite{secli2019theory}, and we will study it more quantitatively in section \textbf{3.6}.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.65]{chapters/recap_1D.png}
    \caption{Elementary excitation spectrum of the lasing mode as a function of the wavevector $k=k_y-k_{yo}$. (a) Zoom on the edge mode dispersion. The black marker indicates the lasing mode. (b) Second derivative of the edge mode dispersion. The black marker indicates the value of the $a_2$ coefficient. (c)-(j) Real and imaginary part of the elementary excitation spectrum as a function of the wave vector k. On the imaginary spectrum, the reservoir mode is not shown as it lays at a high negative value.
    System parameters: $k_{y0}= 2.2987$, $w_0/J = 1.8406$, $a_1/J= -1.3167 $, $a_2/J= -0.5665$, $a_3/J= 0.2609$, $a_4/J = 0.1709$, $\sigma/J = 0$, $\gamma/J= 0.1$, $P=1.25 \gamma$. (c),(d) $g=0$ and $\frac{\gamma_R}{\gamma}= +\infty$ i.e. adiabatic approximation. (e),(f) $g=0$ and $\frac{\gamma_R}{\gamma}= 3$. (g),(h) $g=0.01$ and $\frac{\gamma_R}{\gamma}= +\infty$. (i),(j) $g=-0.01$ and $\frac{\gamma_R}{\gamma}= +\infty$.
    }
    \label{fig3.2}
\end{figure}

 Fig. \ref{fig3.2}(e),(f) show the influence of a slow reservoir on the dynamic of the system. The Golstone mode remains basically the same. The branches on the edges of the imaginary part that come close to the instability threshold $Im(w)=0$ are at high $k$, thus it highlights the necessity of a momentum dependent loss rate . In Fig. \ref{fig3.2}(g)-(j), we compare the influence of the sign of a non-linearity. We find a result consistent with \cite{baboux2018unstable}, which is that stability of the system is ensured provided that the non-linearity ($g$ in our case) has the same sign as the effective mass ($sign(m^{eff}= sign(a_2)$ in our case).




\section{Elementary excitations in the adiabatic approximation}

When $\gamma_R \gg \gamma$, doing the adiabatic approximation as in Chapter \textbf{2} Section \textbf{2}, (\ref{eq:3.1}) reads:

\begin{equation}\label{eq:3.4}
    i\frac{\partial \psi_n}{\partial t} = [w_0 + TF^{-1}[\epsilon(k)](n)\circledast + g|\psi_n|^2 + i(\frac{\chi P^{eff}}{1+\beta |\psi_n|^2} - \gamma) ] \psi_n
\end{equation}

where $\beta = \frac{R}{\gamma_R}$,  $P^{eff} = \beta P_{eq\ 1D}$ and $\chi = (1-i\frac{g_R}{R})$.


This time, the density uniform steady-state (SS) solution reads $\psi_n(t) = \psi^0 e^{-i\mu_T t}e^{i k_{y,0}n}$ where $\psi^0 = \sqrt{\frac{1}{\beta}(\frac{P_{eff}}{P^{eff}_{th}}-1)}$ and $\mu_T = w_0 + g|\psi^0|^2 + \frac{g_R}{R}\frac{P^{eff}}{1+\beta |\psi_0|^2}$. It is reached above the pump threshold $P^{eff}_{th} = \gamma$. Using the same ansatz $\psi_n(t) = \psi^0(1 + \delta \psi_n(t)) e^{-i\mu_T t}e^{i k_{y,0}n}$ with $\delta \psi_n \ll 1$ as previously and passing to fourier space, we get the matricial equation:

\begin{equation}\label{eq:3.5}
i\frac{\partial }{\partial t}&       
\begin{pmatrix} 
        \delta\psi_k \\ 
        \delta\psi_{-k}^{\ast} \\
      \end{pmatrix} 
      = \\
    \begin{pmatrix}
    \epsilon(k) -i\chi \Gamma + \mu & \mu - i\chi \Gamma \\
    -\mu - i\chi^* \Gamma & -\epsilon(-k)^* -i\chi^* \Gamma - \mu
    \end{pmatrix}
    \begin{pmatrix} 
        \delta\psi_k \\ 
        \delta\psi_{-k}^{\ast} \\
      \end{pmatrix} 
\end{equation}

where $\Gamma = \gamma(1-\frac{\gamma}{P_{eq\ 1D}}) = \gamma(1-\frac{P_{th}}{P})$.

Taking $\mu' = \mu - \frac{g_R \Gamma}{R}$, the matrix can be rewritten explicitly as:

\begin{equation}\label{eq:3.6}
    (a_1 k + a_3 k^3)\mathbb{1}
     +
         \begin{pmatrix}
    a_2 k^2 + a_4 k^4 -\frac{i\Gamma}{2} + \mu' & \mu' - \frac{i\Gamma}{2} \\
    -\mu' - \frac{i\Gamma}{2} & -a_2 k^2 - a_4 k^4 -\frac{i\Gamma}{2} - \mu'
    \end{pmatrix}
\end{equation}

In this form, we recognize the second term to be the same as in \cite{chiocchetta2013non} with a free particle dispersion equals to $a_2 k^2 + a_4 k^4$ and a relabelled $\mu'$. Thus the double branched excitation spectrum reads: 
\begin{equation}\label{eq:3.7}
  w_{\pm} = a_1 k + a_3 k^3 - i\Gamma \pm \sqrt{(a_2 k^2 + a_4 k^4)(a_2 k^2 + a_4 k^4 + 2\mu') - \Gamma^2} 
\end{equation}


The main result that we can draw from this approximation is twofold. 
First, the odd orders of the dispersion do not have any influence on the stability of the system (their contribution is real) thus the theory we derive is analytically the same as for a condensate of polaritons in a planar cavity \cite{wouters2007excitations, baboux2018unstable, chiocchetta2013non}.
Second, for $\mu'=0$, the small $k$ dynamic of the Goldstone mode is proportional to $- a_2^2 k^4 $, that is very slow since it is of the forth order and the prefactor $a_2$ is small compared to $J$ due to the strong linear behaviour of the dispersion at the lasing point. This confirms the statement made in the general part.  




\newpage
\section{Application 1: instabilities in S. Longhi, Y. Kominis, and V. Kovanis, Europhysics Letters 122, 14004 (2018)}

In this section, we want to apply our formalism to a recent article \cite{longhi2018presence} that claims that 2D topological laser are not stable in presence of a slow reservoir (class-B laser).

\textit{System and results of the article: }

Their system of study is a square Harper-Hofstadter lattice with flux $\theta = 1/4$, and with pumping on the whole contour of the lattice through a reservoir. The main difference with (\ref{eq:2.3}) and (\ref{eq:2.4}) is that the loss rate is not the same in the bulk as on the edge, and that there is an output coupler in one corner of the lattice. The time evolution of the classical field amplitude $\psi_{m,n}$ in this system is:

\begin{equation}\label{eq:3.8}
\begin{split}
        i\frac{\partial \psi_{m,n}(t)}{\partial t} = &-J[\psi_{m+1,n} +     \psi_{m-1,n} + e^{-2\pi i \theta m}\psi_{m,n+1} + e^{+2\pi i     \theta m}\psi_{m,n-1}] \\
     &+  i ( \sigma (N_{m,n} - 1)-\gamma_p ) (1+i\alpha) \psi_{m,n} \mathbb{1}_{(m,n) \in  \mathcal{P}}  
     - \gamma \psi_{m,n} \mathbb{1}_{(m,n) \notin  \mathcal{P}}
     - \gamma_{out} \psi_{0,0} \mathbb{1}_{(m,n)= (0,0)}
\end{split}
\end{equation}

where the reservoir density $N_{m,n}$ is defined only on the contour ($(m,n) \in  \mathcal{P}$)and is determined by the rate equation:

\begin{equation}
      \frac{\partial N_{m,n}}{\partial t} = P - \gamma_R N_{m,n} + 2\gamma_R (N_{m,n}-1)|\psi_{m,n}|^2) 
\end{equation}

where $j$ is the coupling constant between the sites, $\sigma$ is the amplification term, $\gamma_p$ is the loss rate on the edge, $\alpha$ is the linewidth enhancement factor (equivalent to our $g_R$), $\gamma$ is the loss rate in the bulk, $\gamma_{out}$ is the loss rate due to the output coupler, $P$ is the pump, $\gamma_R$ is the loss rate in the reservoir, $\mathbb{1}$ the indicator function and $\mathcal{P}$ indicates the perimeter of the lattice.

The main result of this article is that for relevant experimental parameters, starting from a small random noise, the lasing on the edge is stable when the ratio $\frac{\gamma_R}{\gamma_p} \gg1 $, and become unstable when  $\frac{\gamma_R}{\gamma_p} \ll 1$, as can be seen in Fig. \ref{fig3.3}.

\begin{figure}[H]   
    \centering
\includegraphics[scale=0.85]{chapters/longhi_transition.png}

   \caption{ Transient switch-on dynamics of the topological insulator laser made of $12 \times 12$ sites. Time is normalized to the cavity photon lifetime $\frac{1}{\gamma_p}$ (i.e. $\tau = t\gamma_p$). Parameter values are: $\theta= 1/4$, $J= 5 ns^{-1}$,  $\alpha=3$, $\gamma_p= 5J$, $\sigma= 96 J$, $\gamma= 0.5J$, $\gamma_{out}= 1J$, $P/\gamma_R= 1.0433$ and  $\gamma_R= 5\gamma_p$ in (a) (virtual limit of class-A
laser), $\gamma_R= 0.01 \gamma_p$ in (b) (class-B laser).
The pump rate $P/\gamma_R= 1.0433$ is chosen very close to its threshold value. Left panels show the normalized intensity distribution $|a_{m,n}|^2$ in the lattice at final time [$t= 10^4/\gamma_p = 0.4 \mu s$ in (a) and $t= 10^5/\gamma_p = 4 \mu s$ in (b)]. Right panels show the temporal evolution of the field intensity at the vertex sites A (output coupler) and B. From \cite{longhi2018presence}}
    \label{fig3.3}
\end{figure} 


\textit{1D gGPE model:}

We now want to use our 1D gGPE model and see if we can capture this transition between stable to unstable. Before all, we do some approximations to be able to use it.

First we perform a 1D approximation on the square geometry. We thus end up with a rectangle. Due to the topological resistance to spatial deformation, we claim that the properties of the edge mode are the same in the square geometry as in a circular one. So we come back in this way to the geometry we studied since the beginning. Note that doing the 1D approximation, we are de facto get rid of the question of the different loss rates inside the bulk and on the edge. We also remove the output coupler for simplicity, which allows us to keep a translational invariant system.

To get the coordinates ($E/J$, $k_y$) of the lasing state, we launch a simulation of the system with the parameters of \cite{longhi2018presence} in the cylinder geometry. Finally we compute the elementary excitations spectrum of the system, which is showed in Fig. \ref{fig3.4}.

\begin{figure}[H]   
    \centering
\includegraphics[scale=0.65]{chapters/LKK_1D.png}

   \caption{Elementary excitations spectrum of the lasing state as a function of the wavevector $k=k_y-k_{yo}$ from the 1D model.
    System parameters: $k_{y0}= -0.9195$, $w_0/J = -2.0869$, $a_1/J= 1.2310 $, $a_2/J= 0.6179$, $a_3/J= -0.2138$, $a_4/J = -0.1567$, $\theta= 1/4$, $J= 5 ns^{-1}$,  $\alpha=3$, $\gamma_p= 5J$, $\sigma= 96 J$, $ \gamma_p^{(2)} = 0.014 J$, $P_{th}= 1.0465 \gamma_R$, $P/\gamma_R= 1.0433$. (a),(b) Real and imaginary part of the spectrum for $\frac{\gamma_R}{\gamma_p}= 5$. (c),(d) Same for $\frac{\gamma_R}{\gamma_p}= 0.01$. 
    }
    \label{fig3.4}    
\end{figure} 

These figures are in good qualitative agreement with the observation of \cite{longhi2018presence}. Indeed in Fig. \ref{fig3.4} (b), that corresponds to a fast reservoir, the system is stable with no mode with positive imaginary value, while in Fig. \ref{fig3.4} (d) that corresponds to a slow reservoir, the system becomes dynamically unstable. Actually, this behaviour is well known with non-equilibrium condensates \cite{wouters2007excitations}, and this proves that these results extend to topological lasers.

Finally, we can discuss what are the key ingredient to observe this behaviour. Indeed, the role of the reservoir is obviously fundamental, as its dynamics is the parameter that drives this transition from stable to unstable. But it is important to say that this transition take place provided there is a non-zero non-linear term, as the parameter $\alpha$ in this case, that corresponds to interactions between particles of the condensate and of the reservoir. Note that in the case of an interaction between the particles of the condensate, the same transition would be observed. When there are no interactions, the system remains stable whatever the speed of the reservoir is (in the 1D model. In the real 2D model, the situation is more complex, as we will see in Chapter \textbf{6}).

(QUE POURRAIT ON AJOUTER POUR ETRE UN PEU PLUS QUANTITATIF ? le seuil ?)



\section{Application 2: ultraslow relaxation time in Secli and al.}

In this section we want to explain the ultraslow relaxation time observed in \cite{secli2019theory}.

\textit{System and results of the article:}

This article has been made by a former student of the team, and his work constitutes the basis of our present work, also the system in this article is very similar to what we have done so far.

It is a square Harper-Hofstadter lattice with flux $\theta = 1/4$ pumped on the whole contour. The pump is taken in the adiabatic approximation so the reservoir is eliminated. There are no interactions and an uniform loss rate, so it is the simplest driven-dissipative system possible. The time evolution of the classical field amplitude reads:

 \begin{equation}
     i\frac{\partial \psi_{m,n}(t)}{\partial t} = -J\Bigg[\psi_{m+1,n} + \psi_{m-1,n} + e^{-2\pi i \theta m}\psi_{m,n+1} 
      + e^{+2\pi i \theta m}\psi_{m,n-1}\Bigg] + \Bigg[ i\Big(\frac{P^{eff}}{1+\beta |\psi_{m,n}|^2} - \gamma \Big) \Bigg] \psi_{m,n}    
\end{equation}

where the parameters are the same as defined in (\ref{eq:2.2}) and (\ref{eq:3.4}).

One of the main result of this article is obtained when the system is let free to evolve to a steady-state after an initial random perturbation. A lasing steady-state in an edge mode is quickly obtained, but in top of it a small perturbation is still present and is damped on a time scale longer than any time scale in the system, namely $\gamma$ or $\frac{L}{v_g}$ which corresponds to the approximate round-trip time around the cavity ($L$ is the perimeter of the cavity and $v_g$ the group velocity of the edge mode).


\begin{figure}[H]   
\begin{minipage}[t]{0.4\textwidth}
This phenomena is illustrated in Fig. \ref{fig3.5}, where we can see the evolution of the intensity profile on one side of the square for increasing time (normalized to a round trip). This clearly shows that the relaxation of the perturbation is very slow.
\end{minipage}
\begin{minipage}[t]{0.6\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=1.2]{chapters/relat_int_var_secli.png}}
 
\end{minipage}
   \caption{Cuts of the intensity distribution along the bottom side of the square at times (from top to bottom) $\gamma t = 4385, 5165, 5945, 6720, 7500 $
    }
   \label{fig3.5}    
\end{figure}


\textit{1D gGPE model:}

Section 3.1 and 3.2 already paved the way for a qualitative explanation of this phenomena. Indeed it was noted that the small $k$ dynamic of the Goldstone mode is very slow, which means that a perturbation around the lasing frequency is damped very slowly. We now want to check that our 1D model is also able to give quantitative predictions.

\begin{figure}[H]   
    \centering
\includegraphics[scale=0.8]{chapters/round_trip.png}
   \caption{ (a) Evolution of the normalized maximal intensity of the perturbation as a function of the number of round trips in a cylindrical geometry. (b) Comparison of the imaginary part of the elementary excitation spectum between a simulation and the 1D model.
    System parameters: $k_{y0}= 2.2089$, $w_0/J = 1.9562$, $a_1/J= -1.2115 $, $a_2/J= -0.6277$, $a_3/J= 0.2041$, $a_4/J = 0.1548$, $\theta= 1/4$, $\mu'/J = 0$, $\gamma/J= 0.1$, $\beta= 0.01$, $\gamma^{(2)}_+/J= 0.014$, $\gamma^{(2)}_-/J= 0.022$, $N_x=11$, $N_y=128$, adiabatic approximation 
    }
    \label{fig3.6}   
\end{figure} 

Like in the previous section, we work in a cylindrical geometry, after having checked that this geometry also exhibits an ultraslow relaxation time for noise (Fig. \ref{fig3.6} (a)). The procedure is the following: we let the system evolve until it reaches the steady-state, and until any perturbation is damped up to the noise limit of the programming device. Then we introduce a little perturbation at a wavector close to the lasing one and let the system evolve. At each time step after the perturbation, we can calculate the space fourier transform of the system, that shows the time evolution of the intensity of each wavevector of the perturbation. For a given wavevector, we assume this evolution to be an exponential decay (which is consistent with simulations), and we fit it to get the slope. This last quantity actually corresponds to the imaginary value of the elementary excitations spectrum at a given wavevector. This allows us to do a direct comparison between our 1D model and a simulation. The result of a such comparison is given in Fig. \ref{fig3.6} (b). It clearly shows a very good agreement between the 1D and the simulation, which confirms that the ultraslow relaxation is due to the slow Goldstone mode around $k=0$. Note also that in order to reproduce well the large $k$ dynamic of the excitations, we had to introduce two different momentum dependent loss rates, one for each branch. 


\begin{figure}[H]   
\begin{minipage}[t]{0.4\textwidth}
 For completeness, the same simulation has been carried out with a smaller lattice, such that there is no mode inside the Goldstone branch. The result is showed in Fig. \ref{fig3.7} and clearly shows that in this case the damping time of the perturbation is much quicker.
\end{minipage}
\begin{minipage}[t]{0.6\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.4]{chapters/round_trip_fast_decay.png}}

\end{minipage}
   \caption{Evolution of the normalized intensity of the perturbation as a function of the number of round trips in the cavity.
    System parameters: $k_{y0}= 2.2440$, $w_0/J = 1.9144$, $\theta= 1/4$, $\mu/J = 0$, $\gamma/J= 0.1$, $\beta= 0.01$, $N_x=11$, $N_y=42$, adiabatic approximation
    }
    \label{fig3.7}    
\end{figure}





\newpage

\section{Application 3: Correlation functions}

In this section, we want to use our 1D gGPE formalism in order to assess the spatial coherence of a lasing state, namely to calculate the spatial correlation functions. 

Up to now, we considered only the deterministic dynamic of the system, namely the dissipation part. But to calculate the spatial correlations of the system, we need to re-introduce the fluctuations. This can be done by simply adding noise to the RHS of the Bogoliubov equation (\ref{eq:3.5}), which allows to compute the steady-state correlations in fourier space:

\begin{equation}
    n^{ss}_k = \langle \psi_k \psi^{*}_k \rangle = 2\pi |\psi^0|^2 \delta(k) + \langle \delta \psi_k \delta \psi^{*}_k \rangle
\end{equation}

where the former term describes the lasing state and the latter the fluctuations.


For simplicity sake, we will compute the correlations in the adiabatic approximation, and follow the procedure of \cite{chiocchetta2013non} that did a similar calculation in the case of a non-equilibrium BEC. The main difference with this work is that we add here odd-derivative terms in the dispersion. 


(CE CALCUL SERA MIT EN APPENDICE SUREMENT)
\textit{Stochastic terms:}

We add a white noise stochastic process $dW(n,t)$ and $dW^{*}(n,t)$, locally correlated in time and space following,

\begin{equation}
    \langle dW(n,t)dW^*(n',t') \rangle = 2D\delta_{n,n'} \delta(t-t') dt
\end{equation}

\begin{equation}
    \langle dW(n,t)dW(n',t') \rangle = 0
\end{equation}

\begin{equation}
    \langle dW^*(n,t)dW^*(n',t') \rangle = 0
\end{equation}

which gives in the fourier domain,

\begin{equation}
    \langle dW_k(t)dW_{k'}^*(t') \rangle = 2\pi 2D\delta_{k,k'} \delta(t-t') dt
\end{equation}

\begin{equation}
    \langle dW_k(t)dW_{k'}(t') \rangle = 0
\end{equation}

\begin{equation}
    \langle dW_k^*(t)dW_{k'}^*(t') \rangle = 0
\end{equation}

Finally (\ref{eq:3.5}) becomes a set of Ito stochastic coupled equations,

\begin{equation}\label{eq:4}
i&       
\begin{pmatrix} 
        d\delta\psi_k \\ 
        d\delta\psi_{-k}^{\ast} \\
      \end{pmatrix} 
      = \\
    \begin{pmatrix}
    \epsilon(k) -\frac{i\Gamma}{2} + \mu' & \mu' - \frac{i\Gamma}{2} \\
    -\mu' - \frac{i\Gamma}{2} & -\epsilon(-k) -\frac{i\Gamma}{2} - \mu'
    \end{pmatrix}
    \begin{pmatrix} 
        \delta\psi_k \\ 
        \delta\psi_{-k}^{\ast} \\
      \end{pmatrix} dt
      +
     \begin{pmatrix} 
        d W_k \\ 
        -d W_{-k}^{\ast} \\
      \end{pmatrix}     
\end{equation}

Formally, we have an equation of this type,

\begin{equation}
    i d\mathbf{v}_k(t) = \mathbb{A}_k \mathbf{v}_k(t)dt + \mathbb{B}d\mathbf{W}_k(t)
\end{equation}

where $\mathbb{B} = \begin{pmatrix}
        -i & 0 \\
        0  & i\\
\end{pmatrix}$

whose formal solution is

\begin{equation}
    \mathbf{v}_k(t) = e^{-i\mathbb{A}_k t} \mathbf{v}_k(0) + \int_0^t e^{-i\mathbb{A}_k (t-\tau)} \mathbb{B} d\mathbf{W}_k(\tau)
\end{equation} 

From this expression we can easily compute the average, using Ito's isometry,

\begin{equation}\label{eq:3.22}
    \langle \mathbf{v}_k(t) \mathbf{v}^{\dagger}_{k'} (t') \rangle = e^{-i\mathbb{A}_k t} \langle \mathbf{v}_k(0) \mathbf{v}^{\dagger}_{k'} (0)  \rangle e^{-i\mathbb{A}^{\dagger}_{k'} t'} + 2\pi 2D \delta_{kk'} \int_0^{min(t,t')}d\tau e^{-i\mathbb{A}_k (t-\tau)} \mathbb{B} \mathbb{B}^{\dagger} e^{-i\mathbb{A}^{\dagger}_k (t'-\tau)}
\end{equation}

Now we can simplify our problem thinking of the form of the $\mathbb{A}_k$ matrix. Indeed, 

\begin{equation}
  \mathbb{A}_k = \epsilon_O(k) \mathbb{1} + \begin{pmatrix}
    \epsilon_E(k) -\frac{i\Gamma}{2} + \mu' & \mu' - \frac{i\Gamma}{2} \\
    -\mu' - \frac{i\Gamma}{2} & -\epsilon_E(-k)^* -\frac{i\Gamma}{2} - \mu'
    \end{pmatrix} =  \epsilon_O(k) \mathbb{1} + \mathbb{A}'_k
\end{equation}

where $\epsilon_O(k)$ ($\epsilon_E(k)$) is the part of the dispersion with odd (even) terms.

It is fundamental to note that the $\mathbb{A}'_k$ matrix is the one that describes a normal non-equilibrium condensate. Indeed, the $\epsilon_O(k) \mathbb{1}$ part of $\mathbb{A}_k$ simplifies in (\ref{eq:3.22}) appearing only as the prefactor $e^{-i\epsilon_O(k)(t-t')}$, which disappears at equal times.

Thus we end up with exactly the same analytic expression for the correlation as in the case of a non-equilibrium BEC. According to the result of \cite{chiocchetta2013non}, the steady-state correlations of the field are:

\begin{equation}
     n^{ss}_k = 2\pi |\psi^0|^2 \delta(k) + \frac{D}{\Gamma}\Bigg[\frac{\mu'^2 + \Gamma^2}{\epsilon_E(k)(\epsilon_E(k) + \mu')} + 1\Bigg]
\end{equation}

In this last expression, it has to be noted that the term $\frac{D}{\Gamma}$ is UV divergent. This is actually an artefact of the model, and is regularized when adding the momentum dependent loss term $\gamma_{tot}(k)= \gamma - i\gamma^{(2)}k^2 $. But since we are mostly interested in the low-k dynamics of the system, it is not necessary to add it here.

\textit{Long range order:}

The steady-state correlation function gives access to the one-time spatial correlation function:

\begin{equation}
    G(n) = \langle \psi^*_n \psi_0 \rangle = \int \frac{dk}{2\pi} n^{ss}_k e^{ikn}
\end{equation}

According to the Penrose-Onsager Criterion, a BEC exists when the correlation function converges to a finite (non zero) value when $n \to \infty$. In our case, it is straightforward to see that the correlation function do not converge in the IR limit, since $\frac{\mu'^2 + \Gamma^2}{\epsilon_E(k)(\epsilon_E(k) + \mu')} \underset{0^+}{\sim} \frac{1}{k^2}$ if $\mu' \neq 0$ ($\underset{0^+}{\sim} \frac{1}{k^4}$ if $\mu'=0$).

This means that the assumption we made that the fluctuations are small is not valid since they diverge, so in other words the assumption that most of the particles are in the condensed/lasing state is wrong. This means that we need to apply a more sophisticated theory able to take into account for large fluctuations, which is the goal of the next section.


\section{Density-phase Bogoliubov theory}

It is known for equilibrium BEC that they cannot exist in low dimension (in 2D without an harmonic trap and in 1D) due to the Mermin-Wagner theorem. But it is still possible to get a transition to a quasi-ordered state, namely a Kostelitz-Thouless transition. The description of the fluctuations of such quasi-ordered states requires a specific approach called \textit{density_phase Bogoliubov theory} \cite{moracastin, popov}. This formalism has also been successfully extended to non-equilibrium condensates \cite{chiocchetta2013non, wc2006}, and the question now is whether the fact to have a dispersion with odd-derivative terms affects these previous result, or if we will get the same behaviour as in the previous section. 

The density-phase Bogoliubov theory corresponds to  expending the wavefunction as:

\begin{equation}\label{eq:3.25}
    \psi_n(t) = \sqrt{n_0 + \delta n_n(t)} e^{-i\theta_n(t)} e^{-i\mu_Tt}
\end{equation}

where $\delta n_n(t) \ll n_0$ and $\theta_n(t)$ are real functions. 


\textit{Bogoliubov matrix:}

Linearizing (\ref{eq:3.25}), we get $\psi_n (t)= \sqrt{n_0}(1 + \frac{\delta n_n(t)}{2n_0} + i \theta_n (t))$

Then, injecting into the gGPE (\ref{eq:3.5}) and taking the real and imaginary part at the first order, we get

\begin{equation}
\centering
\left \{
        \begin{array}{ll}
        \partial_t N_n = -2\Gamma N_n - a_1 \partial_n N_n - a_2 \partial_n ^2 \theta_n + a_3 \partial_n ^3 N_n + a_4\partial^4_n \theta_n\\
        \partial_t \theta_n = -2\mu' N_n - a_1 \partial_n \theta_n + a_2 \partial_n ^2 N_n + a_3 \partial_n ^3 \theta_n - a_4 \partial^4_n N_n
    \end{array}
    \right.
\end{equation}

where $N_n(t) = \frac{\delta n_n (t)}{2n_0}$.

Passing into fourier space, we get

\begin{equation}\label{eq:3.27}
    \frac{d}{dt}      
     \begin{pmatrix} 
        N_k \\ 
        \theta_k 
      \end{pmatrix}(t)
      = 
      \mathbb{B}_k
      \begin{pmatrix} 
        N_k \\ 
        \theta_k 
      \end{pmatrix}(t) 
\end{equation}

where $\mathbb{B}_k$ is the Bogoliubov matrix

\begin{equation}
     \mathbb{B}_k=
     \begin{pmatrix} 
        -2\Gamma -i(a_1 k +a_3 k^3) & a_2 k^2 + a_4 k^4\\ 
        -2\mu' - a_2 k^2 - a_4 k^4 & -i(a_1 k +a_3 k^3)
      \end{pmatrix}
      =
      -i \epsilon_O(k) \mathbb{1} + 
      \begin{pmatrix} 
        -2\Gamma  & \epsilon_E(k)\\ 
        -(2\mu' + \epsilon_E(k)) & 0
      \end{pmatrix}
\end{equation}

\textit{Stochastic terms:}

We add a white noise $dW^N_n(t)$ on the density and $dW^{\theta}_n(t)$ on the phase, assuming that they are not correlated. Thus we have:

\begin{equation}
    \big \langle dW^N_n(t)dW^N_{n'}(t')  \big \rangle = 2D_N \delta(t-t') \delta_{nn'}dt
\end{equation}

\begin{equation}
    \big \langle dW^{\theta}_n(t)dW^{\theta}_{n'}(t')  \big \rangle = 2D_{\theta} \delta(t-t') \delta_{nn'}dt
\end{equation}

\begin{equation}
    \big \langle dW^{N}_n(t)dW^{\theta}_{n'}(t')  \big \rangle = 0
\end{equation}

Identifying $dW^{N}$ ($dW^{\theta}$) to the real (imaginary) part of the noise associated to $\delta \psi_n(t) = \sqrt{n_0} ( \delta N_n(t) + i \theta_n(t))$, it is straightforward to show that the diffusion coefficients are related between each other as

\begin{equation}
    D_N = D_{\theta} = \frac{D}{2n_0}
\end{equation}

where $D$ is the diffusion coefficient of the standard Bogoliubov expansion.


In Fourier space, the noise correlations become

\begin{equation}
    \big \langle dW^N_k(t)dW^N_{k'}(t')^*  \big \rangle = 2\pi2D_N \delta(t-t') \delta_{kk'}dt
\end{equation}

\begin{equation}
    \big \langle dW^{\theta}_k(t)dW^{\theta}_{k'}(t')^*  \big \rangle = 2\pi2D_{\theta} \delta(t-t') \delta_{kk'}dt
\end{equation}

\begin{equation}
    \big \langle dW^{N}_k(t)dW^{\theta}_{k'}(t')^*  \big \rangle = 0
\end{equation}

Finally, adding noise to (\ref{eq:3.27}), we get the stochastic system

\begin{equation}
     d      
     \begin{pmatrix} 
        N_k \\ 
        \theta_k 
      \end{pmatrix}
      = 
      \mathbb{B}_k
      \begin{pmatrix} 
        N_k \\ 
        \theta_k 
      \end{pmatrix} dt 
      +
      \begin{pmatrix} 
        dW^N_k \\ 
        dW^{\theta}_k 
      \end{pmatrix}
\end{equation}

\textit{Resolution:}

Applying Ito's lemma then averaging, we get the system

\begin{equation}
\centering
\left \{
        \begin{array}{lll}
        d\langle N_k N_k^* \rangle = 2 \epsilon_E(k) \langle \theta_k N_k^* \rangle dt  - 4\Gamma \langle N_k N_k^* \rangle dt + 2\pi2D_N dt \\
        d\langle \theta_k N_k^* \rangle = -(\epsilon_E(k) + 2\mu')\langle N_k N_k^* \rangle + \epsilon_E(k)\langle \theta_k \theta_k^* \rangle dt- 2\Gamma  \langle \theta_k N_k^* \rangle dt\\
        d\langle \theta_k \theta_k^* \rangle = -2(\epsilon_E(k) + 2\mu')\langle \theta_k N_k^* \rangle dt + 2\pi2D_{\theta}dt
    \end{array}
    \right.
\end{equation}

It is fundamental to note that these equations are independent on $\epsilon_O$. This means that here again there is no difference between our system and a non-equilibrium condensate. Thus we can take directly the result from \cite{chiocchetta2013non} and apply it to our case:


\begin{equation}
    \langle \delta n_k \delta n_{k'}^* \rangle = \delta_{kk'} \frac{2n_0 D}{\Gamma} \bigg( 1-\frac{\mu'}{\epsilon_E(k) + 2\mu'} \bigg)
\end{equation}

\begin{equation}\label{eq:3.39}
    \langle \delta \theta_k \delta \theta_{k'}^* \rangle = \delta_{kk'} \frac{D}{2n_0 \Gamma} \bigg( 1+\frac{\mu'}{\epsilon_E(k)+ 2\mu'}  + \frac{2(\mu'^2 + \Gamma^2)}{\epsilon_E(k) (\epsilon_E(k) + 2\mu')}\bigg)
\end{equation}

\begin{equation}
    \langle \delta n_k \theta n_{k'}^* \rangle = \delta_{kk'} \frac{D}{\epsilon_E(k) + 2\mu'} 
\end{equation}

\textit{Spatial coherence}

Still on the path of \cite{chiocchetta2013non}, neglecting the fourth order term $a_4 k^4$, we can find an analytic expression for the spatial coherence length of our lasing state.

A the fist order, the correlation length is

\begin{equation}
    G(n) = \langle \psi_n(t) \psi_{0}^*(t) \rangle \approx n_0 \langle e^{-i(\theta_n(t) - \theta_{0}(t)} \rangle \approx n_0 e^{-\frac{G_{\theta}(n)}{2}}
\end{equation}

where the last equality is derived taking in account the gaussian statistics of the noise.

The computation of the correlation function of the phase $\theta_n(t)$ is made in \cite{chiocchetta2013non} by passing (\ref{eq:3.39}) into fourier space. The result is the following:

\begin{equation}
    G_{\theta}(n) =  \bigg[ \bigg(\frac{\xi}{\xi_0(\mu')} \bigg)^3 \frac{n}{\xi} + \bigg(\frac{\xi}{\xi_0(0)} \bigg)^3 (e^{-\frac{|n|}{\xi}}-1) \bigg] \underset{|n| \ll \xi}{\approx} \bigg[ \bigg(\frac{\xi}{\xi_0(\mu')} \bigg)^3 \frac{n}{\xi} + \bigg(\frac{\xi}{\xi_0(0)} \bigg)^3 \frac{n^2}{\xi^2} \bigg]
\end{equation}

where $\xi= \sqrt{\frac{1}{4\mu' m}}$ is the healing length and $\xi_0 (\mu') = \Big( \frac{n_0 \Gamma}{4m^2 D (\mu'^2 + \Gamma^2)} \Big) ^{\frac{1}{3}}$.

From this expression we can distinguish two regimes:

\begin{itemize}
    \item if $\frac{\xi}{\xi_0} \ll 1$ then $G(n) \approx e^{-\frac{|n|}{l_1}}$ where $l_1= \frac{2n_0 \mu' \Gamma }{mD(\mu'^2 + \Gamma^2)}$. In this regime the decay is exponential. It corresponds to a system with strong interactions and highly pumped.
    
    \item if $\frac{\xi}{\xi_0} \gg 1$ then $G(n) \approx e^{-\frac{n^2}{l_2^2}}$ where $l_2= 2\sqrt{\frac{\xi_0^3(0)}{\xi}} = 2\sqrt{\frac{n_0 \mu'^{1/2}}{2m^{3/2}D\Gamma}}$. In this regime the decay is now Gaussian. It corresponds to a regime with weak interactions or close to a point with infinite effective mass ($\frac{\partial^2 w}{\partial k^2}=0$ in Fig. \ref{fig3.2} (b). It is in practice difficult to lase in such a point).
\end{itemize}

Finally, it has to be noted that this result is valid only for an interacting system ($\mu' \neq 0$). When there are no interactions, the linearization to first order is not correct anymore and further non-linear phenomena have to be taken into account. In the case of non-equilibrium condensate, it has led to show that the evolution equation for the phase belongs to the KPZ universality class \cite{gladilin2014spatial}. Similar results are expected in our case and are under investigation currently in the team.

\textit{Comparison with simulation:}

to be done

especially, the role of a big effective mass on the coherence length.

==> chapters/chapter061.tex <==
\chapter{Addition of a reservoir}

In this chapter, we want to compare the 1D and 2D model when we add a reservoir to the system. From the 1D model, we know that in the absence of non-linear interactions, no instabilities are expected.

\section{1D-2D comparison}

For simplicity sake, we consider a system with  $\gamma/J=0.1$, $\beta = \frac{R}{\gamma_R} = 0.01$, $g, g_R=0$, $P = 1.25\frac{\gamma}{\beta}$, $k_{y,0} =-0.9195 $.

The procedure for the simulations is the following: as adding a reservoir makes the computation much longer than in the adiabatic approximation, we re-use every time the previous SS as an initial condition. It is also more stable against noise. So we start our simulation by calculating the SS for a fast reservoir $\gamma_R/\gamma = 100$ and then decrease this ratio. Note that changing the relaxation time of the reservoir will change the SS reservoir density, but not the density of the particles in the system. 

\textit{Results}:

The results of this simulation in the range of reservoir relaxation time $\frac{\gamma_R}{\gamma} = 100$ (i.e. quasi adiabatic) to $\frac{\gamma_R}{\gamma} = 0.1$ (i.e. class-B laser) are displayed in Fig. \ref{fig6.1}. It is clear that the 1D and 2D models are in very good agreement in the full range of parameters of this simulation. 


\section{Ultraslow reverse chirality damping}

When starting the system with a very slow reservoir from a random noise, we observe that the system is not able to reach a stead-state on a reasonable time scale, as showed in Fig. \ref{fig6.2} (a).

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.55]{chapters/low_gr_start_full.png}
    \caption{Time (a) and Fourier (b) evolution of an edge site when starting from a small random noise. 
    System parameters: $\gamma/J= 0.1$, $\beta= 0.01$? $\frac{\gamma_R}{\gamma} = 1$, $g, g_R=0$, $P= 1.25\frac{\gamma}{\beta}$, $\gamma^{(2)}/J= 0.014$, $N_x=31$, $N_y=41$. The white background between the dashed lines in (b) indicates the gaps.
    }
    \label{fig6.2}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[scale=0.75]{chapters/recap_gr.png}
    \caption{Comparison between the 1D and the 2D models elementary excitations spectrums varying the relaxation time of the reservoir $\frac{\gamma_R}{\gamma}$. 
    System parameters: $k_{y,0} = -0.9195$, $\mu_T/J = -1.939$, $a_1/J= 1.2310 $, $a_2/J= 0.6179$, $a_3/J= -0.2138$, $a_4/J = -0.1566$,$\beta= \frac{R}{\gamma_R} = 0.01$, $\gamma/J= 0.1$, $P= 1.25\frac{\gamma}{\beta}$, $\gamma^{(2)}/J= 0.014$, $N_x=31$, $N_y=41$.
    (a)-(h) Real and imaginary part of the elementary excitation spectrum for the 1D (red) and 2D (black) model as a function of the wavevector $k=k_y - k_{y,0}$ for decreasing values of the relaxation time of the reservoir $\frac{\gamma_R}{\gamma}$. The zoom is made around $k=0$ in the relevant part of the 1D model. 
    (a),(b) $\frac{\gamma_R}{\gamma} = 100$, corresponding approximately to the adiabatic regime.
    (c),(d) $\frac{\gamma_R}{\gamma} = 10$. (e),(f) $\frac{\gamma_R}{\gamma} = 1$.
    (g),(h) $\frac{\gamma_R}{\gamma} = 0.1$.
    }
    \label{fig6.1}
\end{figure}







This fact is in contradiction with the simulation ran in the last section, because no instability was retrieved. Making the fourier transform of Fig. \ref{fig6.2} (a) gives further insight on this phenomena. Indeed, in Fig. \ref{fig6.2} (b), we can see that the modes competing for lasing are situated in the topological gaps, but none gap is seeming to win the mode competition. 


\begin{figure}[H]   
\begin{minipage}[t]{0.5\textwidth}
The problem becomes eventually clear when looking at the elementary excitations spectrum calculated in the last section for the same reservoir speed, as shown in Fig. \ref{fig6.3}. We see on this figure that reverse chirality modes are getting very close from the instability threshold. However, contrary to the similar behaviour got with a non linearity, the modes do not cross the threshold when $\gamma_R$ is lowered, but tend to get closer and closer to $Im(w/J)=0$. 
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.85]{chapters/gr_10.png}}
\end{minipage} 

   \caption{Imaginary part of the elementary excitation spectrum for the lasing point \{ $k_{y,0} = -0.9195$, $\mu_T/J = -1.939$\} as a function of the wavevector $k= k_y - k_{y,0}$. Same parameters as Fig. \ref{fig6.2}.}
    \label{fig6.3}   
\end{figure} 

This means that when letting the system evolve freely from a small random noise, the modes loosing the mode competition which are situated in the other gap are damped on a time scale that is extremely long, such that the system is not able to reach a SS on a computable time, mimicking an instability. 

Going further in the investigation about this phenomena, we computed the elementary excitation spectrum for a slow reservoir but with a higher pump intensity ($P= 5.25 \frac{\gamma}{\beta}$. The result is shown in Fig. \ref{fig6.4}. In this picture, we can see that the amplitude modes of reverse chirality went down compared to Fig. \ref{fig6.3}. It means that increasing the pump helps the system to suppress gain to the reverse chirality modes. It is thus a very different mechanism involved compared to the instabilities arising form the addition of non-linear interactions. 


\begin{figure}[H]   
\begin{minipage}[t]{0.5\textwidth}
In this picture, we can see that the amplitude modes of reverse chirality went down compared to Fig. \ref{fig6.3}. It means that increasing the pump helps the system to suppress gain to the reverse chirality modes. It is thus a very different mechanism involved compared to the instabilities arising form the addition of non-linear interactions.
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.85]{chapters/small_gamr_big_P.png}}
\end{minipage} 

   \caption{Imaginary part of the elementary excitation spectrum at high pump intensity ($P= 5.25 \frac{\gamma}{\beta}$ as a function of the wavevector $k= k_y - k_{y,0}$. Other parameters are the same as Fig. \ref{fig6.2}.}
    \label{fig6.4}   
\end{figure} 



Finally, we can think of the results released in \cite{longhi2018presence}. Indeed, in this case the pump intensity is low ($P= 1.0006 P_{th}$), but we claimed in Chapter \textbf{3} Section \textbf{5} that the instabilities are due to the non-linear interaction.
More information are given in the article about the modes responsible for the instability of the system. In Fig. \ref{fig6.5}, a picture from the article shows the different unstable cycles found in presence of weak disorder of resonance frequencies on each site ($w_{ref}$ with the notation of Chapter \textbf{2} Section \textbf{1}). The inset containing power spectrum must be read knowing that the $0$ frequency correspond to the frequency of the lasing mode in Fig. \ref{fig3.3} (a). Thus the frequencies involved in the cycles are situated withing the gap where lasing is possible (it is not possible in the other gap since the non-linear interaction has opposite sign to the effective mass), excepted for Fig. \ref{fig6.5} (e), where in addition to parasite frequencies in the lasing gap, there are also some frequencies in the other topological gap. The fact that most of the time the instability arises from modes in the lasing gap is consistent with the elementary excitations we calculated with the 1D model. Further, the fact that in some cases the reverse chirality modes play a role means that their imaginary part must lay rather close to the instability threshold, consistent with what has been evidenced in this section. 



\section{Conclusion}

In this chapter, we first demonstrated that the elementary excitations at small $k$ are well predicted by the 1D model. However, we discovered an unexpected phenomena which cannot be captured with this model. It consists in the ultraslow decay of modes situated in the opposite gap to the lasing mode, which is increased as the dynamic of the reservoir is slowed down. Then increasing the pump intensity helps to restore a efficient suppression of these modes. Finally, the influence of this new phenomena with the observations of \cite{longhi2018presence} was discussed, concluding that this effect is present but not dominant in this case. 


\begin{figure}[H]
    \centering
    \includegraphics[scale=1.4]{chapters/LKK_recap.png}
    \caption{Same as Fig.\ref{fig3.3}, but with disorder of resonance frequencies. The panels, from (a) to (e), show different runs corresponding to different realizations of disorder, displaying distinct dynamical behavior. The insets in the left panels show the power spectrum of the temporal laser intensity at site A. In (e), the spectral peaks at higher frequencies (at around $\approx 3 GHz$) is ascribed to beating of counter propagating chiral edge modes. In 30 runs, steady-state oscillation after initial transient is observed in 4 runs (i.e. less than $20\% $ times). The most probable outcome is the one in panel (a) (stable periodic limit cycle).
    }
    \label{fig6.5}
\end{figure}



==> chapters/chapter07.tex <==
\chapter{Conclusions}



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.75]{chapters/recap_gr.png}
    \caption{Comparison between the 1D and the 2D models elementary excitations spectrums varying the relaxation time of the reservoir $\frac{\gamma_R}{\gamma}$. 
    System parameters: $k_{y,0} = -0.9195$, $\mu_T/J = -1.939$, $a_1/J= 1.2310 $, $a_2/J= 0.6179$, $a_3/J= -0.2138$, $a_4/J = -0.1566$,$\beta= \frac{R}{\gamma_R} = 0.01$, $\gamma/J= 0.1$, $P= 1.25\frac{\gamma}{\beta}$, $\gamma^{(2)}/J= 0.014$, $N_x=31$, $N_y=41$.
    (a)-(h) Real and imaginary part of the elementary excitation spectrum for the 1D (red) and 2D (black) model as a function of the wavevector $k=k_y - k_{y,0}$ for decreasing values of the relaxation time of the reservoir $\frac{\gamma_R}{\gamma}$. The zoom is made around $k=0$ in the relevant part of the 1D model. 
    (a),(b) $\frac{\gamma_R}{\gamma} = 100$, corresponding approximately to the adiabatic regime.
    (c),(d) $\frac{\gamma_R}{\gamma} = 10$. (e),(f) $\frac{\gamma_R}{\gamma} = 1$.
    (g),(h) $\frac{\gamma_R}{\gamma} = 0.1$.
    }
    \label{fig4.4}
\end{figure}



\section{Fast relaxation of a perturbation}

In the last chapter, we saw that the ultraslow relaxation time is due to the presence of quantified modes in the zone where the Goldstone mode is flat. As with the set of parameters of reference this flat zone is large, this behaviour is observed for lattices of length $N_y \approx 100$. However in presence of non-linearities ($\mu' \neq 0$), the small $|k|$ dynamic of the Goldstone mode is expected to be $\prop k^2$ namely way faster, dramatically shortening the size of the flat zone, as illustrated in Fig. \ref{fig5.2} (the 2D model confirming the guess from the 1D model). In this case, an ultraslow relaxation time of a perturbation is still likely to exist but requires way bigger lattice sites along $N_y$, and is thus considered as suppresses in our case.

==> chapters/fourre_tout.tex <==
\section{1D cylindrical model}

As we see in Fig. \ref{fig3.1} (b), the relevant part of the imaginary part of the elementary excitation spectrum in concentrated in the zone around the lasing mode. This zone is smaller than the gap, so only involves edge modes of the same branch, that propagate in the same direction along the edge in real space. This makes the system behaving as if it was 1-dimensional. 

We thus wrote a 1D equation of motion for a lasing edge mode. We did it by projecting the 2D equations (\ref{eq:4.1}),(\ref{eq:4.2}) on the $y$-axis by mean of the eigenvectors of the bare HH model. The exact derivation of the equation is let in Appendix \ref{appendixA}. Finally, the equation of evolution of a lasing edge mode $\psi_n(t)$ reads:


\begin{equation}\label{eq:3.1}
      \left \{
\begin{array}{l}
\begin{split}
    i\frac{\partial \psi_n}{\partial t}  =  TF^{-1}[\epsilon(k_y)] \circledast \psi_n  + g TF^{-1}[G(k_y)] & \circledast [|\psi_n|^2\psi_n] + g_R TF^{-1}[G(k_y)] \circledast  [N_n \psi_n]\\
    & + i\bigg( R\ TF^{-1}[G(k_y)] \circledast [N_n \psi_n] - \gamma \psi_n \bigg)
    \end{split}\\
    \psi_{N_y} = \psi_{0} \ \forall m
\end{array}
\right.
\end{equation}

where the reservoir density is determined by the rate equation

\begin{equation}\label{eq:3.2}
      \left \{
\begin{array}{l}
      \frac{\partial N_{n}}{\partial t} = P - (\gamma_R + R|\psi_n|^2)N_{n} \\
      N_{N_y} = N_{0} \ \forall m
\end{array}
\right.
\end{equation}

and $\epsilon(k_y)$ is the dispersion of the edge modes in a given gap, $TF^{-1}$ denotes the inverse Fourier transform, $\circledast$ the convolution product, $g$ the strength of the interaction between 2 particles in the lasing mode, $g_R$ is the interaction strength of the interaction between a particle in the lasing mode and a particle in the reservoir, R is the amplification term, $\gamma$ is the on-site loss rate, $\gamma_R$ is the reservoir loss rate, $P$ the uniform pump and $G(k_y)$ corresponds to the intensity overlap between an edge mode of the bare HH Hamiltonian and the pumped edge. 

\textbf{Caution:} this derivation required several approximations (see Appendix \ref{appendixA}). First this model is relevant only to look at the physics inside a gap, since all other modes than the ones inside a given gap are removed. Second, it remains valid only when the non-hermitian gain/loss term is small, which can be written as $\frac{P \gamma}{\Delta w_{gap}} \ll 1$ where $\Delta w_{gap}$ is the size of the topological gaps. As a safety check, note that  $\frac{P \gamma}{\Delta w_{gap}} \approx 0.08$ with the parameters of reference.


 \section{Overlap function and lasing threshold}

\begin{figure}[H]   
\begin{minipage}[t]{0.5\textwidth}
In Fig. \ref{fig3.2}, we see the shape of the $G(k_y)$ function for the edge states along $x=0$ of the bottom gap. At this point, the most important thing to see is that the overlap is never equals to 1, due to the penetration of the wavefunction in the bulk. It explains why the lasing threshold can never be equal to $\gamma$. Moreover, it allows to calculate in a simple manner the threshold. 
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.75]{chapters/gain.png}}
\end{minipage} 

   \caption{Intensity overlap between the edge modes of the bottom gap of the bare HH Hamiltonian indexed by the quantum number $k_y$ and the edge ($x=0$). }
    \label{fig3.2}   
\end{figure} 

Indeed, let us suppose that we want to reach a density uniform steady-state $\psi_n(t)= \psi^0 e^{-i(\mu t - k_{y,0} n)}$ with a reservoir adiabatically eliminated. We thus have that $G(k_y) TF[N_n \psi_n] = G(k_y) N^0 \psi^0 \delta(k_y - k_{y,0})$ so  $TF^{-1}[G(k_y)] \circledast [N_n \psi_n] = G(k_{y,0}) N^0 \psi_n$. The gain/loss term in (\ref{eq:3.1}) then reads $i\Big(\frac{\beta G(k_{y,0}) P}{1+\beta |\psi^0|^2} - \gamma \Big)\psi_n$ which shows clearly that the threshold corresponds to:

\begin{equation}
     P^{eff}_{th}(k_{y,0})= \frac{\gamma}{ G(k_{y,0})}  
\end{equation}

since the intensity is zero at threshold by continuity. As an example, if we calculate the threshold at the maximum value of the overlap (blue dashed line in Fig. \ref{fig3.2}), we retrieve the threshold value that we found in Fig. \ref{fig2.2}. We also find again that the system will tend naturally (if not forced with a seed) to lase in modes in the middle of the gap, where the overlap is maximal.



\section{Elementary excitations in the general case}\label{chap3sec6}

A density uniform steady-state $\psi_n(t) = \psi^0 e^{-i\mu t}e^{i k_{y,0}n}$  where $\psi^0 =
\sqrt{\frac{1}{\beta}(\frac{P}{P_{th}(k_{y,0})}-1)}$ (we can choose the phase so that this term is real),  $N_n(t)=N^0=\frac{P^{eff}_{th}(k_{y,0})}{R}$ and  $\mu = \epsilon(k_{y,0}) + g G(k_{y,0})|\psi^0|^2 + g_R G(k_{y,0}) N^0$  is reached above the pump threshold.



The elementary excitation spectrum is calculated by linearizing (\ref{eq:3.1}) and (\ref{eq:3.2}) around this SS taking the ansatz $\psi_n(t) = \psi^0(1 + \delta \psi_n(t)) e^{-i\mu t}e^{i k_{y,0}n}$ and $N_n(t) = N^0 (1 + \delta N_n(t))$ with $|\delta\psi_n| , |\delta N_n| \ll 1$. Keeping only terms to first order in $\delta \psi_n$ and $\delta N_n$, and Fourier transforming the spatial coordinate we obtain the motion equations in a matricial form:

\begin{equation}\label{eq:3.3}
i\frac{\partial }{\partial t}&       
\begin{pmatrix} 
        \delta\psi_k \\ 
        \delta\psi_{-k}^{\ast} \\
        \delta N_k
      \end{pmatrix} 
      = \\
     \mathcal{L}_k
    \begin{pmatrix} 
        \delta\psi_k \\ 
        \delta\psi_{-k}^{\ast} \\
        \delta N_k
      \end{pmatrix} 
\end{equation}

where 

\begin{equation}
     \mathcal{L}_k = 
     \begin{pmatrix}
    \epsilon^1(k) + \mu_L(k) + i\gamma^1(k) + \mu^1(k) & \mu_L(k)  &  \mu_R(k) + i \gamma G_N(k)\\
    -\mu_L(-k) & -\epsilon^1(-k) - \mu_L(-k) + i\gamma^1(-k) - \mu^1(-k) & -\mu_R(-k) + i \gamma G_N(-k)\\
    -i \alpha \gamma_R & -i \alpha \gamma_R & -i (\alpha +1) \gamma_R
    \end{pmatrix}
\end{equation}



where $\epsilon^1(k)= \epsilon(k)-\epsilon(k_{y,0})$, $\mu_L= g G(k) |\psi^0|^2$, $\mu_R = g_R G(k) N^0 = \frac{g_R \gamma \mu_L}{\alpha \gamma_R}$, $\mu^1(k)=  (g|\psi^0|^2 + g_R N^0)(G(k) - G(k_{y,0}))$, $G_N(k)=\frac{G(k)}{G(k_{y,0})}$, $\gamma^1(k)= \gamma [G_N(k) - 1]$ and $\alpha = (\frac{P}{P_{th}}-1)$.

\vspace{0.25 cm}

Diagonalizing this matrix for each k gives us the elementary excitation spectrum. Taking the typical microscopic parameters introduced in Section \ref{secref}, the full dispersion around the lasing mode and the full $G$ function, we can make a first check of the relevance of this 1D model by comparing its results to the 2D one. This is showed in Fig. \ref{fig3.4}, where we can see that the agreement between the 2 models is nearly perfect.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.7]{chapters/comparaison_1D_2D_reference.png}
    \caption{Real (a) and imaginary (b) part of the elementary excitations spectrum for the 2D model (black dots) and the general 1D model (red dots).
    }
    \label{fig3.4}
\end{figure}


In Appendix \ref{appendixB}, we went further in the checking of the agreement between the 2 models, by comparing in a systematic way the agreement when tuning the main parameters. The agreement found is in most cases perfect. When the non-linearities are turned on, the shape of the branches outside the splitting zone (for the imaginary part) is modified but correspond to information that is not of interest. The important part situated around the lasing mode is still well captured by the 1D model. Also, a "cooking recipe" is found in order to make the condition $\frac{ P \gamma}{\Delta w_{gap}} \ll 1$ more flexible. It consists in neglecting the function $G(k_y)$, only keeping the zero order term $G(k_{y,0})$. This value is then replaced by the value $\frac{\gamma}{P_{th}^{effective}(k_{y,0})}$ where the threshold value is found using the procedure of Chapter \ref{chap1} Section \ref{chap1sec3}. 


Finally, we showed in this section and the previous ones that the 1D cylindrical model reproduces correctly the behaviour of the system around a topological edge mode. The main strength and interest of this model is that it allows to calculate the elementary excitations of the 2D system directly from the microscopic parameters, without requiring to compute the steady-state of the system. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This phenomenon can eventually be predicted quantitatively with the 1D effective model, adding only the contribution of the edge modes of the other gap. Between $[-\pi, 0]$, we take into account the dispersion of the branch where is the lasing mode, and between $[0, \pi]$ the one of the edge modes in the other gap. The result of this cooking recipe is showed in red in Fig. \ref{fig4.3} (a) and is found to be in perfect agreement with the expected result. 

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.65]{chapters/large_k_enhancement_and_high_pump_recipe.png}
   \caption{Imaginary part of the elementary excitations spectrum around the lasing edge mode for  $\frac{\gamma_R}{\gamma} =25$ and (a) $P= 1.25\gamma$, (b) $P= 2.25\gamma$.
   Dark (red) lines correspond to computations with the 2D (1D effective) model.}
    \label{fig4.3}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{2D problem:}

Equation of evolution of the field amplitude on each site with PBC along the $y$-axis:

\begin{equation}\label{eq1}
\left \{
\begin{array}{l}
\begin{split}
i\frac{\partial \psi_{m,n}}{\partial t}(t) = -J[\psi_{m+1,n} + \psi_{m-1,n} &+ e^{-2\pi i \theta m}\psi_{m,n+1} 
      + e^{+2\pi i \theta m}\psi_{m,n-1}] \\
      & + [ g|\psi_{m,n}|^2 + g_R N_{m,n} + i(R N_{m,n} - \gamma) ] \psi_{m,n}   
\end{split}\\ 
            \frac{\partial N_{m,n}}{\partial t}(t) = P \delta_{m,0} - (\gamma_R + R|\psi_{m,n}|^2)N_{m,n} \\
      N_{m,N_y} = N_{m,0} \ \forall m
\end{array}
\right.
\end{equation}

with $\psi_{m,N_y} = \psi_{m,0} \ \forall m$ and $N_{m,N_y} = N_{m,0} \ \forall m$.


Given the translationnal invariance of the system, we can decompose in Fourier space a solution of the set of equations of the $\psi_{m,n}$ as:

\begin{equation}\label{eq3}
    \bra{x,k_y}\ket{\psi} = \psi(x,k_y) =   \overline{\psi}(k_y)\phi_{k_y}(x)
\end{equation}

\ul{ with the normalization $\phi_{k_y}(0)=1$.}

Nb: from now, we will use indifferently {$x \iff m$}, {$y \iff n$} and {$\int dk_y \iff \sum_{k_y} $}.

\textbf{Goal:}

We want to write the equation of evolution of a lasing edge mode in a simple way. The propagation of a chiral edge mode is unidirectional along the edge of the system, corresponding to the $y$-axis in our case. We thus want to eliminate the $x$ variable by projecting the equation on the $y$-axis, and get a 1D equation of evolution of $\overline{\psi}(y) = \int d_ky e^{ik_y y} \overline{\psi}(k_y)$.




\textbf{Projector:}

We want a projector such that:

\begin{equation}\label{eq4}
    \bra{\phi, y}\ket{\psi} = \overline{\psi}(y)
\end{equation}

It is then straightforward to check that the projector $\ket{\phi, y}$ defined by:

\begin{equation}
    \ket{\phi, y} = \int dk_y e^{ik_y y}  \ket{\phi, k_y}
\end{equation}

where 

\begin{equation}
    \bra{x,k_y'}\ket{\phi, k_y}= \frac{\phi_{k_y}(x)\delta_{k_y,k_y'}}{\sum_x |\phi_{k_y}(x)|^2}
\end{equation}

fills the condition (\ref{eq4}).

\textbf{Approximation:}

As we do not dispose of the solutions of the non-hermitian problem (\ref{eq1}),(\ref{eq2}), we do not have the exact expression of the $\phi_{k_y}$.

To circumvent this problem, we rather project onto the state $\ket{\phi^{HH}, k_y}$ where the $\phi^{HH}_{k_y}$ functions correspond to the one of the bare HH model, without taking into account for the non-hermitian part.

Then we make the fundamental approximation which consists in neglecting the non-hermitian contribution to the $\phi_{k_y}$ when the shift of the spectrum due to the non-hermitian terms is negligible, i.e.:

\begin{equation}
    \bra{\phi^{HH}, k_y}\ket{\phi, k_y}= \bra{\phi^{HH}, k_y}\ket{\phi^{HH}, k_y} + \mathcal{O}(\frac{P \gamma}{\Delta w_{gap}} )
\end{equation}

where $\Delta \omega_{gap}$ is the size of the topological gaps, which is the good energy scale to compare to the non-hermitian contribution.

\textbf{Projection of the motion term:}

We want to calculate:

\begin{equation}
    \mel{\phi^{HH}, y}{H^{HH}}{\psi}
\end{equation}

As $\ket{\psi^{HH}}$ is a solution of the HH Hamiltonian corresponding to an edge mode, we have:

\begin{equation}
    H^{HH}\ket{\phi^{HH}, k_y} = \epsilon(k_y) \ket{\phi^{HH}, k_y}
\end{equation}

where $\epsilon(k_y)$ is the dispersion of the edge modes in the branch of study. 

So we end up with:

\begin{equation}
    \mel{\phi^{HH}, k_y}{H^{HH}}{\psi} = \epsilon(k_y) \overline{\psi}(k_y) 
\end{equation}

Thus:

\begin{equation}
    \mel{\phi^{HH}, y}{H^{HH}}{\psi} = TF^{-1}[\epsilon(k_y)]\circledast \overline{\psi}(y)
\end{equation}

\textbf{Reservoir equation:}

This term depends on the reservoir. We then first remark that (\ref{eq2}) has a non zero SS only for $m=0$. Thus we make the approximation that $N_{m,n} = \overline{N}_{n}\delta_{m,0}$.

This simplifies the problem since $\psi(0,y) = \int dk_y e^{ik_y y} \overline{\psi}(k_y) \phi_{k_y}(0) = \overline{\psi}(y)$. The reservoir equation thus directly depends on $\overline{\psi}$.

\textbf{Projection of the $N_{m,n}\psi_{m,n}$ term:}

We want to calculate:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{N}\ket{\psi}
\end{equation}

where $\mel{x,y}{\hat{N}}{\psi}= N(x,y)\psi(x,y)$

We have:

\begin{equation}
\begin{split}

    \bra{\phi^{HH}, k_y} \hat{N} \ket{\psi}& = 
    \sum_x \sum_{x'} \int \int dk_y ' dy' \bra{\phi^{HH}, k_y}\ket{x, k_y '}  \bra{x, k_y '}\ket{x', y'} \bra{x', y'}\hat{N} \ket{\psi}\\
    \\
    & = \sum_x \int dy' e^{i k_y y'} \frac{\phi^{HH}_{k_y}(x)}{\sum_x |\phi^{HH}_{k_y}(x)|^2} N(x,y') \psi(x,y')
    = \int dy' e^{i k_y y'} \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \overline{N}(y') \overline{\psi}(y')\\
    \\
    & = \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} TF\Big[\overline{N}(y)\overline{\psi}(y)\Big](k_y)
\end{split}
\end{equation}

So we end up with:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{N}\ket{\psi}
    = TF^{-1}\Bigg[\frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2}\Bigg] \circledast \Big[\overline{N}\overline{\psi}\Big](y)
\end{equation}

\textbf{Projection of the $|\psi_{m,n}|^2 \psi_{m,n}$ term:}

We want to calculate:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{X^2}\ket{\psi}
\end{equation}

where $\mel{x,y}{\hat{X^2}}{\psi}= |\psi(x,y)|^2\psi(x,y)$

We have:

\begin{equation}\label{eq16}
\begin{split}

    \bra{\phi^{HH}, k_y} \hat{X^2} \ket{\psi}& =
    \sum_x \int dy' e^{i k_y y'} \frac{\phi^{HH}_{k_y}(x)}{\sum_x |\phi^{HH}_{k_y}(x)|^2} |\psi(x,y')|^2 \psi(x,y') \\
    & = \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} \phi^{HH}_{k_y}(0) |\psi(0,y')|^2 \psi(0,y')
    + \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} \phi^{HH}_{k_y}(1) |\psi(1,y')|^2 \psi(1,y') + ...
    \\
    & = \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} |\overline{\psi(y')}|^2 \overline{\psi(y')} + \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} \phi^{HH}_{k_y}(1) |\psi(1,y')|^2 \psi(1,y') + ... 
\end{split}
\end{equation}

For a SS of the system (\ref{eq1}),(\ref{eq2}), we measure that the intensity on the second site is typically around $10 \%$ the one of the first one starting from the pumped edge. This means that the second term in the expansion of (\ref{eq16}) is roughly $100$ times smaller than the first one. We thus neglect this contribution, as well as the ones of the further terms in $x$.

We finally end up with:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{X^2}\ket{\psi} = TF^{-1}\Bigg[\frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2}\Bigg] \circledast [|\overline{\psi}|^2\overline{\psi}\Big](y)
\end{equation}

\textbf{Shape of the gain and lasing threshold:}

Our final 1D equation depend on the function $TF^{-1}\Bigg[\frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2}\Bigg]$, where we will write $G(k_y) = \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2}$ from now. We now want to explain in what consists this term.

If we take the normalized (physical) wavevectors $\ket{\phi^{HH}_N, k_y}$ of $H^{HH}$ (such that $H^{HH}\ket{\phi^{HH}_N, k_y} = \epsilon(k_y) \ket{\phi^{HH}_N, k_y} $ with $\bra{\phi^{HH}_N, k_y}\ket{\phi^{HH}_N, k_y} = 1$), then the relation with \ket{\phi^{HH}, k_y} is:

\begin{equation}
    \ket{\phi^{HH}, k_y} = \frac{1}{|\phi^{HH}_{N, k_y}(0)|^2} \ket{\phi^{HH}_N, k_y}
\end{equation}

which means that 

\begin{equation}
    G(k_y) = \sum_x |\phi^{HH}_{k_y}(x)|^2 = \frac{1}{|\phi^{HH}_{N, k_y}(0)|^2}
\end{equation}

We eventually see that the function corresponds to the overlap between a mode and the edge. For the gain term, it means that the gain is not momentum uniform but rather depends strongly on it.


\begin{figure}[H]   
\begin{minipage}[t]{0.5\textwidth}
In Fig. \ref{fig3.2}, we see the shape of the $G(k_y)$ function for the edge states along $x=0$ of the bottom gap. An important thing to see is that the overlap is never equals to 1, due to the penetration of the wavefunction in the bulk. It explains why the lasing threshold can never be equal to $\gamma$. Moreover, it allows to calculate in a simple manner the threshold. 
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \centering
    \raisebox{\dimexpr-\height+\ht\strutbox\relax}{\includegraphics[scale=0.75]{chapters/gain.png}}
\end{minipage} 

   \caption{Intensity overlap between the edge modes of the bottom gap of the bare HH Hamiltonian indexed by the quantum number $k_y$ and the edge ($x=0$). }
    \label{fig3.2}   
\end{figure} 

Indeed, let us suppose that we want to reach a density uniform steady-state $\psi_n(t)= \psi^0 e^{-i(\mu t - k_{y,0} n)}$ with a reservoir adiabatically eliminated. We thus have that $G(k_y) TF[N_n \psi_n] = G(k_y) N^0 \psi^0 \delta(k_y - k_{y,0})$ so  $TF^{-1}[G(k_y)] \circledast [N_n \psi_n] = G(k_{y,0}) N^0 \psi_n$. The gain/loss term in (\ref{eq:3.1}) then reads $i\Big(\frac{\beta G(k_{y,0}) P}{1+\beta |\psi^0|^2} - \gamma \Big)\psi_n$ which shows clearly that the threshold corresponds to:

\begin{equation}
     P^{eff}_{th}(k_{y,0})= \frac{\gamma}{ G(k_{y,0})}  
\end{equation}

since the intensity is zero at threshold by continuity. As an example, if we calculate the threshold at the maximum value of the overlap (blue dashed line in Fig. \ref{fig3.2}), we retrieve the threshold value that we found in Fig. \ref{fig2.2}. We also find again that the system will tend naturally (if not forced with a seed) to lase in modes in the middle of the gap, where the overlap is maximal.

\textbf{Cooking recipe:}

When $\frac{P\gamma}{\Delta \omega_{gap}}$ becomes comparable to 1, the approximation we did to project on the bare HH eigenvectors breaks down. However, as we saw in the previous paragraph the zero order of the $G$ function gives the lasing threshold, and we have an algorithm to calculate the lasing threshold of the full 2D model. We thus can infer the zero order of the $G$ function at high $\frac{P \gamma}{\Delta \omega_{gap}}$ from this new threshold. We then suppose that the shape of the $G$ function remains the same (at least at intermediate $k$, i.e. $|k| \approx 0.75$), so we set:

$G^{cook}(k) = \frac{\gamma}{P^{algo}_{th}(k_{y,0})}\frac{G(k)}{G(k_{y,0})}$. 

\textbf{gGPE:}

The 1D equation of evolution of a lasing edge mode $\psi_n(t)$ eventually reads:


\begin{equation}\label{eq:3.1}
      \left \{
\begin{array}{l}
\begin{split}
    i\frac{\partial \psi_n}{\partial t}  =  TF^{-1}[\epsilon(k_y)] \circledast \psi_n  + g TF^{-1}[G(k_y)] & \circledast [|\psi_n|^2\psi_n] + g_R TF^{-1}[G(k_y)] \circledast  [N_n \psi_n]\\
    & + i\bigg( R\ TF^{-1}[G(k_y)] \circledast [N_n \psi_n] - \gamma \psi_n \bigg)
    \end{split}\\
    \psi_{N_y} = \psi_{0} \ \forall m
\end{array}
\right.
\end{equation}

where the reservoir density is determined by the rate equation

\begin{equation}\label{eq:3.2}
      \left \{
\begin{array}{l}
      \frac{\partial N_{n}}{\partial t} = P - (\gamma_R + R|\psi_n|^2)N_{n} \\
      N_{N_y} = N_{0} \ \forall m
\end{array}
\right.
\end{equation}


This equation is not practical to use in practice due to the several convolutions. So, a brutal approximation which can be made to simplify it a lot is to neglect all the orders of the $G$ function and to keep only the zero one. This amounts to neglect all the momentum dependence of the gain of the system, which is only valid in a narrow window around the lasing mode frequency. However, in Appendix \ref{appendixB}, we can see a comparison of the elementary excitations calculated with this model and with the 2D one and state that this approximation allows for retrieving with fidelity the shape of the Goldstone and Higgs modes. 

Finally, in this approximation, we get a generalized Gross-Pitaevskii Equation (gGPE) \cite{carusotto2013quantum} for the evolution of the field amplitude:

\begin{equation}\label{eq:3.4}
    i\frac{\partial \psi_n}{\partial t} = \Bigg[ TF^{-1}[\epsilon(k_y)](n)\circledast + g G_0 |\psi_n|^2 + g_R G_0 N_n + i\Big(R G_0 N_n - \gamma\Big)\Bigg]\psi_n
\end{equation}

where the reservoir follows the equation,

\begin{equation}
    \frac{\partial N_n}{\partial t} =
    P - \gamma_R (1+R |\psi_n|^2) N_n
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In order to proof further that it is these modes that are involved, we can probe this instability in another way. We take as initial pattern the SS got from a stable simulation with $g=0.01$, that we perturb with a small random noise. We then let evolve with $g=0.055$,  above threshold. We see clearly in Fig. \ref{fig5.6} (a) that the system first want to stabilize in the SS for the new value of $g$ but is unable to damp the growing perturbation. The frequencies involved in this growing perturbation are displayed in Fig. \ref{fig5.6} (b) which confirms that the instability is due to modes in the top gap, thus having a reverse chirality compared to the lasing mode.


\begin{figure}[H]
    \centering
    \includegraphics[scale=0.55]{chapters/instability_g_2.png}
    \caption{Time (a) and fourier (b) evolution of a edge site for $g=0.055$, just above instability threshold . In (b), the white (grey) background stands for the gaps (bulk). 
    }
    \label{fig5.6}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Again, we probe this instability by turning the pump intensity to $P^{ad}= 2.20\gamma$, which is  just above the instability threshold, starting from a stable pattern (SS of the simulation for $g=0.01$ and $P^{ad}= 2.15\gamma$), that we perturb with a random noise. We see in Fig. \ref{fig5.8} (a) that the system reaches the new SS meanwhile the perturbation is growing slowly. At a certain point, the perturbation seems to reach a stable cycle (around $T=3000$). In Fig. \ref{fig5.8} (b), we computed the Fourier transform of the signal on the edge within the time frame in the white zone in (a). This shows that the system is perturbed by two modes symmetrical around the lasing mode, that are gaining in amplitude with time (not shown), and correspond to the ones of Fig. \ref{fig5.7}. In the steady unstable regime, other modes are further excited due to the instability of the bulk modes perturbing the system.



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.60]{chapters/instability_P_g2.png}
    \caption{Time (a) and Fourier (b) evolution of an edge site for $P^{ad}= 2.20\gamma$ and $g=0.01$ just above instability threshold. In (a), the white background between the dashed line corresponds to the time frame on which the Fourier Transform (FT) in (b) is computed. The red horizontal lines in (b) refer to the vertical line in Fig. \ref{fig5.7} (a).
    }
    \label{fig5.8}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Projection of the motion term:}

We want to calculate:

\begin{equation}
    \mel{\phi^{HH}, y}{L^{HH}}{\psi}
\end{equation}

where $L^{HH}$ is the lattice term such that $L^{HH}\ket{\psi} = -J[\psi_{m+1,n} + \psi_{m-1,n} &+ e^{-2\pi i \theta m}\psi_{m,n+1} 
      + e^{+2\pi i \theta m}\psi_{m,n-1}]$

As the $\ket{\psi^{HH}}$ are solutions of the lattice term, and that we limit them to edge modes of the same gap, we have:

\begin{equation}
    L^{HH}\ket{\phi^{HH}, k_y} = \epsilon(k_y) \ket{\phi^{HH}, k_y}
\end{equation}

where $\epsilon(k_y)$ is the dispersion of the edge modes in the branch of study. 

So we end up with:

\begin{equation}
    \mel{\phi^{HH}, k_y}{L^{HH}}{\psi} = \epsilon(k_y) \overline{\psi}(k_y) 
\end{equation}

Thus:

\begin{equation}
    \mel{\phi^{HH}, y}{L^{HH}}{\psi} = TF^{-1}[\epsilon(k_y)]\circledast \overline{\psi}(y)
\end{equation}

\textbf{Reservoir equation:}

This term depends on the reservoir. We then first remark that (\ref{eq1}) has a non zero SS only for $m=0$. Thus we make the approximation that $N_{m,n} = \overline{N}_{n}\delta_{m,0}$.

This simplifies the problem since $\psi(0,y) = \int dk_y e^{ik_y y} \overline{\psi}(k_y) \phi_{k_y}(0) = \overline{\psi}(y)$. The reservoir equation thus directly depends on $\overline{\psi}$.

\vspace{0.75cm}
\textbf{Projection of the $N_{m,n}\psi_{m,n}$ term:}

We want to calculate:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{N}\ket{\psi}
\end{equation}

where $\mel{x,y}{\hat{N}}{\psi}= N(x,y)\psi(x,y)$

We have:

\begin{equation}
\begin{split}
&\bra{\phi^{HH}, k_y} \hat{N} \ket{\psi} = \\
&\sum_x \sum_{x'} \int \int dk_y ' dy' \bra{\phi^{HH}, k_y}\ket{x, k_y '}  \bra{x, k_y '}\ket{x', y'} \bra{x', y'}\hat{N} \ket{\psi}\\
& = \sum_x \int dy' e^{i k_y y'} \frac{\phi^{HH}_{k_y}(x)}{\sum_x |\phi^{HH}_{k_y}(x)|^2} N(x,y') \psi(x,y')\\
&\stackrel{N_{m,n>0} =0}{=} \int dy' e^{i k_y y'} \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \overline{N}(y') \overline{\psi}(y')\\
& = \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} TF\Big[\overline{N}(y)\overline{\psi}(y)\Big](k_y)
\end{split}
\end{equation}

So we end up with:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{N}\ket{\psi}
    = TF^{-1}\Bigg[\frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2}\Bigg] \circledast \Big[\overline{N}\overline{\psi}\Big](y)
\end{equation}


\textbf{Projection of the $|\psi_{m,n}|^2 \psi_{m,n}$ term:}

We want to calculate:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{X^2}\ket{\psi}
\end{equation}

where $\mel{x,y}{\hat{X^2}}{\psi}= |\psi(x,y)|^2\psi(x,y)$

We have:


\begin{equation}\label{eq166}
\begin{split}
\bra{\phi^{HH}, k_y} &\hat{X^2} \ket{\psi} =
\sum_x \int dy' e^{i k_y y'} \frac{\phi^{HH}_{k_y}(x)}{\sum_x |\phi^{HH}_{k_y}(x)|^2} |\psi(x,y')|^2 \psi(x,y')\\
& = \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} \phi^{HH}_{k_y}(0) |\psi(0,y')|^2 \psi(0,y') \\
&+ \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} \phi^{HH}_{k_y}(1) |\psi(1,y')|^2 \psi(1,y') + ... \\
& = \frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} |\overline{\psi(y')}|^2 \overline{\psi(y')} + \\
&\frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2} \int dy' e^{i k_y y'} \phi^{HH}_{k_y}(1) |\psi(1,y')|^2 \psi(1,y') + ... 
\end{split}
\end{equation}



For $k_y$ close to the gain maximum, we measure that the intensity on the second site ($x=1$) is typically around $10 \%$ the one of the first one ($x=0$). This means that the second term in the expansion of (\ref{eq166}.15) is roughly $100$ times smaller than the first one. We thus neglect this contribution, as well as the ones of the further terms in $x$.


We finally end up with:

\begin{equation}
    \bra{\phi^{HH}, y} \hat{X^2}\ket{\psi} = TF^{-1}\Bigg[\frac{1}{\sum_x |\phi^{HH}_{k_y}(x)|^2}\Bigg] \circledast \Big[|\overline{\psi}|^2\overline{\psi}\Big](y)
\end{equation}






